Solving Rubik's Cube via Quantum Mechanics and Deep Reinforcement Learning

Rubik's Cube is one of the most famous combinatorial puzzles involving nearly $4.3 \times 10^{19}$ possible configurations. Its mathematical description is expressed by the Rubik's group, whose elements define how its layers rotate. We develop a unitary representation of such group and a quantum formalism to describe the Cube from its geometrical constraints. Cubies are describedby single particle states which turn out to behave like bosons for corners and fermions for edges, respectively. When in its solved configuration, the Cube, as a geometrical object, shows symmetrieswhich are broken when driven away from this configuration. For each of such symmetries, we build a Hamiltonian operator. When a Hamiltonian lies in its ground state, the respective symmetry of the Cube is preserved. When all such symmetries are preserved, the configuration of the Cube matches the solution of the game. To reach the ground state of all the Hamiltonian operators, we make use of a Deep Reinforcement Learning algorithm based on a Hamiltonian reward. The Cube is solved in four phases, all based on a respective Hamiltonian reward based on its spectrum, inspired by the Ising model. Embedding combinatorial problems into the quantum mechanics formalism suggests new possible algorithms and future implementations on quantum hardware.

==> images/Commentario.tex <==
corners0.png rappresenta l'orientazione iniziale che abbiamo scelto per i corners, le freccine indicano dove punta lo ''spin'' nell'orientazione risolta, cioè dove dev'essere collocata correttamente la faccia del cubetto

edges0.png è uguale al precedente, ma per gli edges

cubies.png dà una semplice panoramica grafica su cosa siano corners ed edges nel Cubo

Abbiamo poi un po' di candidati, per così dire, nel rappresentare le trasformazioni del gruppo:

    Per rappresentare come muta lo stato di momento angolare (cioè la posizione) dei corners, abbiamo:
        cornersladder.png
        L+.png
        corners_rot.png
    
    Invece, per il momento angolare degli edges, abbiamo:
        edges.png
        edgesnew.png
        edgesnew2.png
        edge_rot.png
        

    

